ThreshKnot: Thresholded ProbKnot for Improved RNA Secondary Structure Prediction

RNA structure prediction is a challenging problem, especially with pseudoknots. Recently, there has been a shift from the classical minimum free energy-based methods (MFE) to partition function-based ones that assemble structures using base-pairing probabilities. Two examples of the latter group are the popular maximum expected accuracy (MEA) method and the ProbKnot method. ProbKnot is a fast heuristic that pairs nucleotides that are reciprocally most probable pairing partners, and unlike MEA, can also predict structures with pseudoknots. However, ProbKnot's full potential has been largely overlooked. In particular, when introduced, it did not have an MEA-like hyperparameter that can balance between positive predictive value (PPV) and sensitivity. We show that a simple thresholded version of ProbKnot, which we call ThreshKnot, leads to more accurate overall predictions by filtering out unlikely pairs whose probabilities fall under a given threshold. We also show that on three widely-used folding engines (RNAstructure, Vienna RNAfold, and CONTRAfold), ThreshKnot always outperforms the much more involved MEA algorithm in (1) its higher structure prediction accuracy, (2) its capability to predict pseudoknots, and (3) its faster runtime and easier implementation. This suggests that ThreshKnot should replace MEA as the default partition function-based structure prediction algorithm. ThreshKnot is already available in the widely used RNAstructure software package version 6.2 (released November 27, 2019): https://rna.urmc.rochester.edu/RNAstructure.html

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty *.cls)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs_Threshknot/*.pdf)
figfiles += $(wildcard figs_SI/*.pdf)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

#%.pdf : %.ps
#	ps2pdf $< $@
#	~/local/macscripts/refresh.scpt

#	cd figs; mptopdf *.mp; cd ..

# %.pdf: %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
# 	pdflatex ${*F} #> ${*F}.log
# 	#tail ${*F}.log
# 	@if  grep Citation ${*F}.log ; then \
# 		bibtex ${*F};   \
# 		pdflatex ${*F};      \
# 		bibtex ${*F};   \
# 		pdflatex ${*F}
# 	#fi
# 	#open $@
# #	~/local/macscripts/refresh.scpt


fast: *.tex
	pdflatex main

%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	#pdflatex si
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	pdflatex $<
	#@-/bin/rm -f ${tmp_files}
	#pdfcrop --margin "5 5 5 5" main.pdf
	# open main-crop.pdf

long.bib:	all.bib
	./remove-short.pl all.bib > long.bib


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

paper.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=1 -dLastPage=12 main.pdf

si.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=13 -dLastPage=20 main.pdf




==> alg.tex <==
%\vspace{-0.2cm}

%\subsection*{LinearFold Algorithm}

%We 
%Figures~\ref{fig:overview}B and~\ref{fig:method}
%We present the high-level idea of \linearfold step-by-step, starting from the naive, exhaustive search, version, 
%and gradually improve it to the linear-time version,
%shown in .
%For simplicity purposes and

%Here we first formulate the \linearfold algorithm more formally.

\subsection{Problem Formulation}
\label{sec:formulation}

%% The RNA secondary structure prediction problem can be formalized as follows,
%% using the dot-bracket format to represent structures.
Given an RNA sequence
$\vecx = x_1x_2\ldots x_{n}$,  where each $x_i \in \{\tt{A},\tt{C},\tt{G},\tt{U}\}$,
the secondary structure prediction problem
%$\mathit{f}$ 
aims to find the best-scoring pseudoknot-free structure \vecyhat
%$$ \vecy = y_1y_2\ldots y_{n}, \text{ where } y_i \in \{\md, \ml, \mr\}$$
%(to address pseudoknots, different types of brackets would be required)
by maximizing a scoring function \scorew (e.g., model score or negative free energy) where $\weight$ are the model parameters:
% (or minimum model cost):
\vspace{-0.1cm}
\begin{equation}
  %f(\vecx) =
  \vecyhat = \argmax_{\vecy \in \GEN(\vecx)} \scorew(\vecx, \vecy).
  \label{eq:mfe}
\end{equation}
%\vspace{-0.2cm}
Here $\GEN(\vecx)$ is the set of all possible pseudoknot-free secondary structures for input \vecx of length $n$
\[
%\GEN(\vecx) =
\big\{\vecy \in \{\md, \ml, \mr\}^n \mid \balanced(\vecy), \valid(\vecx,\pairs(\vecy))\big\}
\]
where %$|\vecx|$ is the length of \vecx and
$\balanced(\vecy)$ checks if \vecy has balanced brackets,
and $\valid(\vecx,\pairs(\vecy))$ checks if all pairs in \vecy are valid (CG, AU, GU)
and $\pairs(\vecy)$ returns the set of $(i,j)$ pairs where $x_i$ and $x_j$ form a base pair in \vecy,
e.g.,
$\pairs(\text{``\ml\ml\md\mr\mr''}) = \{(1,5), (2,4)\}$.
See SI for detailed definitions.

%and %$\score$ is the cost function (i.e., free
%energy function), and
%% The two baselines in our study, \contrafold
%% and \viennarnafold, use scoring functions that are very similar  in structure, % scoring functions,
%% but very different in parameters 
%% (the former learns \vecw from data, % in which the free energy
%% %is not revealed,
%% while the latter is based on thermodynamics).

All dynamic programming-based prediction algorithms, including ours, %like previous ones, are based on dynamic programming,
require the scoring function $\scorew(\vecx,\cdot)$ to {\em decompose} to the scorings of smaller structures.
%in order to have efficient computation.
%% For example, the main text (see Fig.~\ref{fig:method}) uses the simplest Nussinov-style scoring function 
%% that factors to each individual base pair and simply counts the number of pairs in a structure:
%% \begin{equation}
%%   \score_{\text{Nussinov}}(\vecx, \vecy; \_) = \# \pairs(\vecy) = \sum_{(i,j)\in \pairs (\vecy)} 1
%%   \label{eq:nussinov}
%% \end{equation}
%% where $\pairs(\vecy)$ returns the list of base pairs in \vecy, e.g.,
%% $\pairs(\text{``\md\ml\ml\md\mr\mr\md''}) = \{(2,6), (3,5)\}$.
%% Note this scoring function does not depend on any model,
For simplicity of presentation,
in the main text we will use a very simple decomposition to individual pairs and unpaired nucleotides:
\begin{equation}
  \scorew(\vecx, \vecy) = \!\!\!\sum_{(i,j)\in \pairs (\vecy)} \!\!\! w_{x_i x_j} + \!\!\!\sum_{i\in \unpaired(\vecy)} \!\!\! \wunpaired
  \label{eq:simple}
\end{equation}
In this framework we can assign different scores for different pairs, % (e.g., $\wgc > \wau > \wgu$)
and incur a penalty for each unpaired nucleotide. % ($\wunpaired < 0$).
For the example in Fig.~\ref{fig:method}, we simply set %$\wcg\!=\!1$, $\wau\!=\!0.5$, $\wgu\!=\!0.1$,
$\wcg\!=\!\wau\!=\!\wgu\!=\!1$
and $\wunpaired\!=\!-0.1$;
therefore, $\scorew(\text{``CCAGG''}, \text{``\ml\ml\md\mr\mr''}) \!=\! 2 \wcg \!+\!\wunpaired \!=\! 1.9$.


In reality, however, the actual scoring functions % $\score$ (scoring structure \vecy on input \vecx by model \vecw) can be
used by \contrafold, \rnafold, and our \linearfold are much more complex,
and they decompose into individual loops.
See SI for details.
%all the model weights are learned from data, instead of the free energy.
%% We conclude
%% the cost decomposition in Fig.~\ref{fig:realdeduct}. 

%% RNA secondary structure prediction is regarded as a challenging problem,
%% that no existing model can score perfectly to match the actual
%% structure with the minimum free energy (or minimum model cost) function, i.e.,
%% {\bf imperfect modeling}.
%% Consider $y^*(\vecx)$ as the actual secondary structure of the given sequence,
%% and an evaluation metric (e.g., PPV, sensitivity) $M$ to
%% calculate accuracy of a set of predicted structures against the actual
%% structures ($M(y,y)=1$), we are likely to have $M(f(\vecx), y^*(\vecx)) < 1$
%% according to the existing results reported(see Fig.\ref{fig:accuracy}).

%% Our proposed \linearfold algorithm can linearize any system with a variant of
%% $(\score,\weight)$, as long as $f(\vecx) = \argmin_{\vecy \in \GEN(\vecx)}
%% \score(\vecx, \vecy; \weight)$ can be 
%% solved in cubic-time by the dynamic programming algorithm.
%% The linearization maintains the same cost function and model $(\score,\weight)$,
%% but the objective function is different, i.e. $f' \neq f$, as we set a series of
%% soft constraints
%% during the beam search, pruning out structures with high cost or high free
%% energy which depends on the given $(\score,\weight)$.
%% Experimental results show that
%% this difference leads to a higher accuracy in linearizing \contrafold and
%% Vienna RNAfold (see Fig.~\ref{fig:accuracy} and Fig.~\ref{fig:beamsize}).

%% Our \linearfold algorithm can ``linearize'' any cubic-time prediction system
%% as long as the scoring function decomposes in a way similar to Eqs.~\ref{eq:nussinov}--\ref{eq:decomp} above.
%% Below we formalize our \linearfold algorithm step by step, % as follows.
%% using the Extended Nussinov model in Eq.~\ref{eq:extended} to strike a balance between simplicity
%% and reality.
%% We will refer to both the high-level illustration in Fig.~\ref{fig:method},
%% and a more formal deductive system in Fig.~\ref{fig:deduction}.

% The basic idea of our proposed

% We propose \linearfold, the first global linear-time RNA secondary structure
% prediction algorithm. 
% The basic idea of linear-time prediction is to predict incrementally from
% left to right,
% %, inspired by human sentence processing. To adapt it to RNA
% %sequences, 
% %we view the problem as incrementally converting the RNA sequence into
% %the dot-bracket format, such that 
% labeling each nucleotide  as unpaired ``{\textbf .}'', opening ``{\textbf (}'',
% or closing ``{\textbf )}''. 
% %% This makes the
% %% dot-bracket format equivalent to the pseudoknot-free RNA secondary structures
% We require this dot-bracket string to be well-balanced as we only consider pseudoknot-free structures
% (to address pseudoknots, different types of brackets would be required. This is left as our future work). 

% the term "exponentially traverse" is strange, I suggest "traverse all possible
% structures in GEN(\vecx), which takes exponenential time
%% 4-step method claim
%\vspace{.25cm}

\input{methodfigure}

%% Without loss of generality, we  sketch our algorithm in Fig.~\ref{fig:method} using the Nussinov model~\cite{nussinov+:1978}: %(maximizing the number of base pairs),
%% for a given RNA sequence, we aim to find the secondary structure in a valid dot-bracket format (Fig.~\ref{fig:overall}B) with the maximum number of base pairs;
%% the case with state-of-the-art thermodynamic and machine learning models are presented in Online Methods and Figs.~\ref{fig:deduction}, \ref{fig:pseudocode}, and \ref{fig:realdeduct}.


\subsection{Idea 0: Brute-Force Search: $O(3^n)$}

The initial idea, introduced in %of \linearfold
Fig.~\ref{fig:overall}B, %of linear-time prediction 
is to scan the RNA sequence left-to-right,
maintaining a {\em stack} along the way, and
performing one of the three actions
(push, skip, or pop)
at each step. % $j$ on nucleotide $x_j$ $(j=1\ldots n)$.
More formally, we denote each {\em state} at step $j$ ($j=0...n$)
as a tuple along with a score $s$:
%\begin{equation}
\[
        \nnitem{\vecy}{\sigma}{j}{s},
\]
%$s = \nitem{{\bm \sigma} | i}{j}\vecy$,
%\end{equation}
where \vecy is the (sub)structure for the prefix $x_1 \ldots x_j$,
and
$\sigma$ is the  stack consisting of unmatched opening bracket positions in \vecy.
%For the Nussinov model, score $s$ is simply the number of pairs in \vecy.
For example, in step 4, if \vecy=``\bml\ml\md\mr'', then $\sigma=[1]$ and $s=0.9$ (see Fig.~\ref{fig:method}A);
note that %for each state, its stack is simply the positions of unpaired open brackets (always shown
we denote open brackets in bold.
%and $s$ is the score of the state.
%% so far
%% where $i$ is the top of the stack, meaning $x_i$ is the last unmatched opening nucleotide. 
%$\vecy$ is the corresponding dot-bracket (sub)sequence up to $x_{j-1}$.
Each state at step $j$ can transition into a subsequent state of step $j\!+\!1$, taking one of the three
actions:
\begin{enumerate}[itemsep=-1mm]
\item \push:
  label $x_{j+1}$ as ``\ml'' for it to be paired with a downstream nucleotide, and pushing $j+1$ on to the stack, % $\sigma$ which becomes $\sigma| (j+1)$,
  notated:
  \[
  \frac{\nnitem{\vecy}{\sigma}{j}{s}}{\nnitem{\vecy\!\circ\!{\text `}\ml{\text '}}{\sigma | (j+1)}{j+1}{s}}
  \]
%which labels the current nucleotide $x_j$ as a left bracket ``{\textbf (}'', 
%putting it on top of the stack;
\item \nskip:
  label $x_{j+1}$ as ``\md'' (unpaired and skipped): %for stack
  \[
  \frac{\nnitem{\vecy}{\sigma}{j}{s}}{\nnitem{\vecy\!\circ\!{\text `}\md{\text '}}{\sigma}{j+1}{s + w_\unpaired}}
  \]
%, which labels $x_j$ as a dot ``{\textbf .}'', leaving the stack unchanged,
%and 
\item \pop:
  label $x_{j+1}$ as ``\mr'', paired with the upstream nucleotide $x_i$
  where $i$ is the top of the stack, and pop $i$
  (if $x_i x_{j+1}$ pair is allowed):
  \[
  \frac{\nnitem{\vecy}{\sigma | i}{j}{s}}{\nnitem{\vecy\!\circ\!{\text `}\mr{\text '}}{\sigma}{j+1}{s+ w_{x_i x_{j+1}}}}
  \]
%, which labels $x_j$ as a right bracket ``{\textbf )}'', 
%if it matches $x_i$
%nucleotide with $x_{\TOP}$, the top of the stack, 
%and popping $i$ from the stack.
\end{enumerate}
%See Fig.~\ref{fig:deduction}(a) for the deductive system.
% labeled dot-bracket sequences ($|y|=j$).
% Then the prediction algorithm
% starts with \(\nitem{\sigma_{\epsilon}}{0}{\epsilon}\), and ends with
% $|\GEN(x)|$ different states,
% \begin{equation}
%   \nitem{\sigma_{\epsilon}}{n}{y} ,y \in \GEN(x).
% \end{equation}
%% Starting at the state \(\nitem{\sigma_{\epsilon}}{0}{\epsilon}\), it takes
%% This algorithm takes $O(3^n)$ time to exhaustively traverse all possible
%% %structures (see the first part of Figure~\ref{fig:method}).
%% structures (see Figure~\ref{fig:method}D1).

%% \vspace{-0.1cm}
%% \begin{enumerate}[itemsep=-1mm]
%% \item {\em skip}: labeling $x_j$ as dot ``\md'', i.e., it is unpaired and {\em skipped}; %for stack
%% %; this is known as the \nskip action;\\
%% \item {\em push}: labeling $x_j$ as open bracket ``\ml'' for it to be paired with a downstream nucleotide, and {\em pushing} $j$ on to the stack; or
%% \item {\em pop}: labeling $x_j$ as close bracket ``\mr'', paired with the upstream nucleotide $x_i$
%% where $i$ is the top of the stack, and {\em pop} $i$.
%% \end{enumerate}
%% \vspace{-0.1cm}
%(opening ``{\textbf (}''),
%% or paired with an upstream nucleotide (closing ``{\textbf )}'').
We start with the init state $\nnitem{\text{`'}}{[\,]}{0}{0}$ and finish with any state $\nnitem{\vecy}{[\,]}{n}{s}$ with an empty stack
(ensuring the output is a well-balanced dot-bracket sequence). % corresponding to a pseudoknot-free secondary structure).
See Fig.~\ref{fig:method}A for an example path for input sequence CCAGG, and Fig.~\ref{fig:method}D for all valid paths.
%% A {\em state} at each step $j$ is a (sub)structure for the prefix input $x_1 ... x_j$; e.g., 
%% ``\md\bml'' and ``\bml\bml'' are two of the possible states for the prefix CC, with [2] and [1,2] being their corresponding stacks.
%% Note that for each state, its stack is simply the positions of unpaired open brackets (shown in bold).


%TODO: explain states

%% and requiring brackets to be well-balanced,
%% as we explore the pseudoknot-free prediction algorithm in this paper which
%% only contains one set of brackets. 
\iffalse
Our \linearfold approach is presented in four steps,
starting from the most naive but easy-to-understand exhaustive search version,
and gradually build it up to the linear-time version,
showing in Fig.~\ref{fig:method}, with the
full deduction system described in Fig.~\ref{fig:deduction} and
Figure~\ref{fig:realdeduct}. 
% \footnote{simplified from the real systems, this figure
% shows an illustration just maximizing the number of pairs: part A
% is illustrating from three selected pathes, and part B is the whole
% demonstration. }
The basic idea of linear-time prediction is to predict incrementally from left
to right,
labeling each nucleotide as dot or bracket (unpaired ``{\textbf .}'', opening ``{\textbf (}'', or closing ``{\textbf )}''.),
and requiring brackets to be well-balanced.
% Thus only three labels are used:
\fi

% The most intuitive way to apply incremental prediction is to start from an
% initial state at the beginning of the sequence, which in each step transition to
% every possible subsequent state by taking one labeling action, until the whole
% sequence is processed. This naive exhaustive incremental prediction is taking an
% exponential $O(3^n)$ time, showing in Figure~\ref{fig:method}~A1/B1. 
% %% not connected between sentences
% A stack $s$ is
% stored in each state to store all the previous unpaired opening positions, and
% thus pair canonicality can be checked when closing a bracket is attempted. 

% In Figure~\ref{fig:method} A1/B1, we show that the

The above procedure describes a naive exhaustive search without dynamic programming
which has exponential runtime
$O(3^n)$, as there are up to three actions per step (see Fig.~\ref{fig:method}D).

%% The RNA secondary structure can be
%% predicted by naive exhaustive incremental prediction, using an exponenential
%% $O(3^n)$ time (see Figure~\ref{fig:method}D).
%% We start from an initial
%% state at the beginning of the sequence, and in each step it can transition to
%% any possible subsequent state by taking one of the three labeling actions. 
%% We also keep a stack $s$ in each state to store all the previous unpaired
%% opening positions, and thus pair canonicality can be checked when closing a
%% bracket is attempted (see Figure~\ref{fig:method}A). 
% The deductive system is described in Figure~\ref{fig:deduction}~(a). 

%We now
Next, Fig.~\ref{fig:method}B
sketches
the two key dynamic programming ideas that speed up
this algorithm to $O(n^3)$ by merging and packing states.
%using two example paths in Figure~\ref{fig:method}B.

\subsection{Idea 1: Dynamic Programming by Merging States with Identical Stacks: $O(2^n)$}

We first observe that different states can have the same stack; for example,
in step 5, both ``\md\ml\md\mr\md'' and ``\ml\ml\md\mr\mr'' have the same empty stack (see Fig.~\ref{fig:method}B, Idea 1);
and in step 4, both ``\bml\md\md\md'' and ``\bml\ml\md\mr'' have the same stack [1] (see Fig.~\ref{fig:method}D).
%% in Figure~\ref{fig:method}B, the two states in the last step, , both have empty stacks,
%% and in Figure~\ref{fig:method}D, in step 4, both 
These states can be merged, because even though they have different histories, going forward they are exactly equivalent.
After merging we save the state with the highest score and discard all others which have no potential to lead to the optimal structure.
More formally, we merge two states with the same stack:
\[
\begin{rcases}
  \nnitem{\vecy}{\sigma}{j}{s}\\
  \nnitem{\vecy'}{\sigma}{j}{s'}
\end{rcases}
\!\!\!\goesto \nitemt{\sigma}{j}{\vecy'', s''} %\maxtwo (\tuple{\vecy, s}, \tuple{\vecy', s'})} %{\tuple{y'', s''}}}
\]
where %$\maxtwo(\cdot, \cdot)$ returns the better tuple along the second dimension, i.e.,
\[
%\maxtwo (\tuple{\vecy, s}, \tuple{\vecy', s'}) =
\tuple{\vecy'', s''} =
\begin{cases}
  \tuple{\vecy, s} & \text{if $s > s'$}\\
  \tuple{\vecy', s'} & \text{otherwise}
\end{cases}
\]

This algorithm is faster but still has exponential $O(2^n)$ time as there are exponentially many different stacks (see Fig.~\ref{fig:method}E).
%% We further apply dynamic programming to this basic version to exploit shared
%% computations, demonstrated in Figure~\ref{fig:method}B(Idea 1).
%% We merge states in the same step if they are sharing the exact
%% same stack, since they would behave exactly the same in the remaining steps except
%% the label history. 
%% This is still exponential ($O(2^n)$) for the exponential number of different
%% stacks.



\subsection{Idea 2: Dynamic Programming by Packing Temporarily Equivalent States: $O(n^3)$}

We further observe that even though some states have different stacks,
they might share the same stack top.
For example, 
in step 2, ``\md\bml'' and ``\bml\bml'' have [2] and [1,2] as their stacks, resp.,
but with the same stack top 2. % (see also Fig.~\ref{fig:method}B).
Our key insight is that two states with the same stack-top
are ``temporarily equivalent'' and can be ``packed'' as they would behave equivalently until the
stack-top open bracket is closed (i.e., matched), after which they ``unpack'' and diverge.
As shown in Fig.~\ref{fig:method}B (Idea 2),
%To be more concrete,
both ``\md\bml'' and ``\bml\bml'' are looking for a ``G'' to match with the stack top $x_2$=``C'',
and can be packed as ``\mq\bml'' with stack [...2] where \mq and ``...'' represent
histories that are not important for now. After skipping the next nucleotide $x_3$=``A'', they become ``\mq\bml\md''
and upon matching the next nucleotide $x_4$=``G'' with the stack-top $x_2$=``C'', they unpack, resulting in ``\md\ml\md\mr'' and ``\bml\ml\md\mr''.

More formally, two states $\nitemt{\sigma | i}{i}{\vecy, s}$ and $\nitemt{\sigma' | i}{i}{\vecy', s'}$ sharing the same stack top can be packed:
\[
\begin{rcases}
  \nitemt{\sigma | i}{i}{\vecy,s}\\
  \nitemt{\sigma' | i}{i}{\vecy',s'}
\end{rcases}
\!\!\!\goesto \nitemt{i}{i}{\bml, 0} %{\tuple{y'', s''}}}
\]
Note that (a) we only need two indices to index the packed state;
(b) we omit the \mq's since they contain no information; and (c) somewhat counterintuitively, the resulting packed state's (sub)structure and score, $\tuple{\bml, 0}$
do not depend on the original states before packing.
More formally, for any packed state $\nitemt{i}{j}{\vecy, s}$,
its \vecy is a substructure only for the substring $x_i ... x_j$,
and its score $s$ is also for that portion only, i.e., $s=\scorew(x_i ... x_j, \vecy)$.
We can grow it by skip
\[
\frac{\nitemt{i}{j}{\vecy, s}}{\nitemt{i}{j+1}{\vecy\circ\text{`\md'}, s+\wunpaired}}
\]
or push actions
\[
\frac{\nitemt{i}{j}{\vecy, s}}{\nitemt{j+1}{j+1}{\bml, 0}}.
\]

The pop action is more involved. If $x_i$ and $x_{j+1}$ match,
we pop $i$, but where can we find the ``previous stack top''? It is {\em not} specified in the packed state.
Therefore, we need to find a state $\nitemt{k}{i-1}{\vecy', s'}$ that combines with the current state:
\[
\frac{\nitemt{k}{i-1}{\vecy',s'} \quad \nitemt{i}{j}{\vecy, s}}{\nitemt{k}{j+1}{\vecy'\circ\vecy\circ\text{`\mr'}, s'+s+w_{x_i  x_{j+1}}}}
\]





%% A key point of \linearfold algorithm is to pack states with different
%% stacks by looking at its stack-top only, which is different from all the previous
%% RNA secondary structure prediction approaches. %% another point: beam search
%% Two states with the same stack-top would behave the same until the
%% top opening bracket is closed, when they would start behaving differently.
%% To achieve this we \textbf{pack} the left states 
%% % (see green arrows in Figure~\ref{fig:method} B/C)
%% and \textbf{unpack} them to split the
%% paths back in a closing-bracket action.
% (see red arrows in Figure~\ref{fig:method} B/C). %% NOT CLEAR!!!
This method (see Fig.~\ref{fig:method}F) %has only $O(n)$ states per step, resulting in
runs in $O(n^3)$ time, because the pop step involve three free indices.
It guarantees to return the optimal-scoring structure. % (i.e., exact search); %\cite{huang+sagae:2010};
%see Online Methods and Figure~\ref{fig:deduction} for details. % and complexity analysis.
%We demonstrate  stack-top packing in Figure~\ref{fig:method}B(Idea 2).
It is adapted from a well-established algorithm in natural language parsing \cite{tomita:1988,huang+sagae:2010}.
Although this $O(n^3)$ runtime is the same as those classical bottom-up ones,
its unique left-to-right nature makes it amenable to linear-time beam search. %beam pruning, it linear-time in practice.



\subsection{Idea 3: Beam Pruning: $O(n)$}

We further employ beam pruning~\cite{huang+:2012},
a popular heuristic widely used in computational linguistics,
to reduce the complexity from $O(n^3)$ to $O(n)$,
but with the cost of exact search.
% Thus we extend it with a beam search framework.
%% need or not?
% Although our dynamic programming algorithm is the of same complexity as 
% traditional algorithms, the key difference is that our new dynamic programming
% algorithm is {\bf incremental} (i.e., left-to-right) instead of  {\bf
%   bottom-up} as in traditional CKY-style algorithms (Nussinov, Zuker, McCaskill,
% etc.), which makes the beam search framework only applicable to our prediction algorithm.
Basically, at each step $j$, we only keep the $b$ top-scoring (lowest-energy) states % $\tuple{i, j}$ 
%by score 
%for each step $j$,
and prune the other, less promising, ones (because they are less likely to be part of the optimal final structure).
This results in an approximate search algorithm in  $O(nb^2)$ time,
depicted in %, which is linear in $n$.
Figure~\ref{fig:method}C and G.
%see pseudocode in Figure~\ref{fig:pseudocode}.
On top of beam search, we further borrow the more advanced technique of cube pruning~\cite{huang+chiang:2005,huang+chiang:2007}
%which is another heuristic widely used in computational linguistics to speed up approximate dynamic programming to
to reduce the runtime to $O(n b\log b)$.
Here the beam size $b$ is a small constant (by default 100) so the overall runtime is linear in $n$.
%Fig.~\ref{fig:beamsize} shows that the search error
We will show that although our linear-time search is approximate, it nevertheless achieves higher overall prediction accuracy than the classical cubic-time exact search methods.
%% generate the best
%% $b$ states, which would take $O(b\log b)$ time.
%Thus the overall running time over a length-$n$ sequence is $O(nb\log b)$, see 

\smallskip
Above we sketched a simplified version of the LinearFold Algorithm.
See SI for the real system.

%% In this way lower-scoring (higher-energy) states are pruned
%% out, and if a
%% structure survives to the end, it must have been one of the top $b$
%% states in every step.
%% This pruning also means that in a pop action, a state $(i,j)$ can combine with at most $b$ states $(k,i)$ from step $i$.
%% Thus the overall time complexity is $O(nb^2)$.
%% %% , i.e., a pop
%% %% action can produce at most $b$ subsequent states.
%% However, instead of generating $b^2$ new states from a pop action, % from a step $j$, 
%% we use \textbf{cube pruning} \cite{huang+chiang:2007} to generate the best
%% $b$ states, which would take $O(b\log b)$ time.
%% Thus the overall running time over a length-$n$ sequence is $O(nb\log b)$, see 
%% See Figure~\ref{fig:method}C(Idea 3)/D4 for beam search.


%% Our algorithm is not only left-to-right incremental, which makes it
%% ``linearizable'', but also more expressive for
%% each state,
%% which can now represent exponential number
%% of prefix secondary structures in the original search space. 
%% As a result, we further employ beam search to reduce the complexity to linear
%% time and linear space (see Figure~\ref{fig:method}C(Idea 3)),
%% keeping a constant number of top-scoring states for each step,
%% and pruning out all the lower-scoring states.
%% Importantly, this requires the surviving substructures to be highly scored at
%% \textbf{each} step, resulting a higher overall accuracy than the exact prediction
%% baselines, especially on long sequences (see next subsection).
%% We further use cube pruning in the packing-unpacking process, resulting our time
%% complexity reduced from $O(nb^2)$ to $O(nb\log b)$ \cite{HuangChiang-iwpt05}.
%% We give more details about our algorithm in Online Methods, and
%% formalize it using ``deductive systems''~\cite{pereira+warren:1983,shieber+:1995} in
%% %actual deductive system is in
%% Figures~\ref{fig:deduction} and~\ref{fig:realdeduct};
% and 
% our actual codebase is available
% at \href{https://github.com/abentu0101/LinearFold}{Github}. \footnote{https://github.com/abentu0101/LinearFold} 
%% Another key point of \linearfold is beam search. 


% impact of beam sizes


\iffalse
\begin{table}[t]
\begin{tabular}{r|rr|r}
memory & \contrafoldmfe & \viennarnafold & \linearfold $b$=100\\
\hline 
%% space & \multicolumn{2}{c|}{$O(n^2)$}                   & $O(nb)$\\
%% \hline       
16G    & 27,500         & 27,500         &             \\
32G    & 32,500         & 32,500         &             \\
\end{tabular}
\smallskip
\caption{Maximum sequence length allowed by different predictors on 
machines with 16G and 32G memory.\label{tab:max}}
\end{table}
\fi

\begin{figure}% [h] % should belong in result.tex
  \centering
  \begin{tabular}{cc}
    % \begin{subfigure}
    %   \centering
    \hspace{-1em}
\raisebox{5.2cm}{\large A}
\hspace{-2.5em}
      \includegraphics[width=.29\textwidth]{figs/scatter_Mathews_hzhang.pdf}
      %\caption{Time vs. sequence length on all sequences in Mathews data.}
    % \end{subfigure}
    &      
      % \begin{subfigure}
      %   \centering
      \hspace{-3em}
\raisebox{5.2cm}{\large B}
      \hspace{-2.4em}
      \raisebox{0.15cm}{\includegraphics[width=.26\textwidth]{figs/rnacentral_hzhang.pdf}}
      %\caption{Time vs. sequence length on all sequences in the RNAcentral data.}
    % \end{subfigure}
    \\[-1.5cm]
    %(a) time: ArchiveII set & \hspace{-4.5em} (b) time: RNAcentral set (log-log)\\[-1.2cm]
    \multicolumn{2}{c}{
\hspace{-1cm}
%\vspace{-1cm}
\raisebox{4cm}{\large C}
\includegraphics[width=.45\textwidth]{figs/mem_log_hzhang.pdf}}\\[-1.5cm]
   %\multicolumn{2}{c}{\hspace{-1cm}(c) memory: RNAcentral set (log-log)}
  \end{tabular}
  \caption{Efficiency and scalability of \linearfold. 
    {\bf A}: runtime comparisons on the ArchiveII dataset
% : running time against sequence length,
    %\linearfoldc (with beam sizes 100 and 50) vs.~
    with the two baselines, \contrafoldmfe and \viennarnafold. %(\linearfoldv have identical running time with \linearfoldc).
    {\bf B}: runtime comparisons on the RNAcentral dataset (log-log).
    {\bf C}: memory usage comparisons (RNAcentral set, log-log).
    \linearfold uses $O(n)$ time and memory, being substantially faster and slimmer than the $O(n^3)$-time, $O(n^2)$-space, baselines on long sequences.
    %% (a) the ArchiveII dataset, while the right one (log-log) uses % a set of 
    %% the RNAcentral data. 
    \label{fig:time}\vspace{-0.3cm}
    %% Each node represents a running example.
    %% The curve in the left figure shows the regression of examples from each algorithm.
  }
\end{figure} % should belong in result.tex


\iffalse
\subsection{Practical Systems}

and they
decompose to individual loops: % as follows:
\begin{equation}
  \begin{split}
 \score_\text{real}(\vecx, \vecy; \weight) = &
 \!\!\!\!\sum_{h \in \text{hairpin\_loops}(\vecy)}\!\!\!\! \score^{\mathrm H}(\vecx, h; \weight)  + \!\!\!\!\sum_{s \in \text{single\_loops}(\vecy)}\!\!\!\! \score^{\mathrm S}(\vecx, s; \weight) \\
 + & \!\!\!\!\sum_{m \in \text{multi\_loops}(\vecy)}\!\!\!\! \score^{\mathrm M}(\vecx, m; \weight) +  \!\!\!\!\sum_{e \in \text{external\_loops}(\vecy)}\!\!\!\!\!\!\!\! \score^{\mathrm E}(\vecx, e; \weight).
\end{split}
\label{eq:decomp}
\end{equation}
The thermodynamic %minimal free energy
model in \viennarna scores %, the score of constructing 
each type of loop %(hairpin, single-branch, multi-branch, and external)
using several feature templates such as
hairpin/bulge/internal loop lengths,
terminal mismatches, helix stacking, helix closing, etc.
%% %the following feature components:\cite{mathews+:1999}
%% \begin{itemize}[itemsep=-1mm]
%% \item %$\score^{\mathrm H}(\cdot,\cdot;\cdot)$,
%% Hairpin loops: hairpin length, terminal mismatch, and special tri-, tetra-, and hexa-loops. 
%% \item %$\score^{\mathrm S}(\cdot,\cdot;\cdot)$,
%% Single-branch loops (including helix stacking as empty loop, and bulge and internal loops):
%% bulge length, internal loop length, internal loop left-right balancing,
%% terminal mismatch, helix stacking, and helix closing.
%% \item %$\score^{\mathrm M}(\cdot,\cdot;\cdot)$,
%% Multi-branch loops: multi-loop base cost, terminal mismatch,
%% left/right dangles, multi paired, and multi unpaired.
%% \item %$\score^{\mathrm E}(\cdot,\cdot;\cdot)$,
%% External loops: left/right dangles, external paired and external  unpaired. 
%% \end{itemize}
The machine-learned model in \contrafold
replaces energies in the above framework with model weights learned from data.

\fi


==> result_bak.tex <==
%\Vspace{0.1cm}
\smallskip

%% TODO: Dezhong: re-write result section starts here

% \vspace{-0.1cm}
\begin{figure}%[h] % should belong in result.tex
  \centering
  \begin{tabular}{cc}
    % \begin{subfigure}
    %   \centering
    \hspace{-1em}
\raisebox{5.4cm}{\large A}
\hspace{-2em}
      \includegraphics[width=.28\textwidth]{figs/scatter_Mathews.pdf}
      %\caption{Time vs. sequence length on all sequences in Mathews data.}
    % \end{subfigure}
    &      
      % \begin{subfigure}
      %   \centering
      \hspace{-3.4em}
\raisebox{5.4cm}{\large B}
      \hspace{-2.4em}
      \includegraphics[width=.267\textwidth]{figs/rnacentral.pdf}
      %\caption{Time vs. sequence length on all sequences in the RNAcentral data.}
    % \end{subfigure}
    \\[-1cm]
    %(a) time: ArchiveII set & \hspace{-4.5em} (b) time: RNAcentral set (log-log)\\[-1.2cm]
    \multicolumn{2}{c}{
\hspace{-1cm}
\raisebox{4cm}{\large C}
\includegraphics[width=.45\textwidth]{figs/mem_log.pdf}}\\[-1.2cm]
   %\multicolumn{2}{c}{\hspace{-1cm}(c) memory: RNAcentral set (log-log)}
  \end{tabular}
  \caption{ 
    A: runtime comparisons on ArchiveII dataset:
% : running time against sequence length,
    \linearfoldc (with beam sizes 100 and 50) vs.~two baselines, \contrafoldmfe \& \viennarnafold (\linearfoldv have identical running time with \linearfoldc).
    B: runtime comparisons on RNAcentral dataset (log-log).
    C: memory usage comparisons (RNAcentral set, log-log).
    %% (a) the ArchiveII dataset, while the right one (log-log) uses % a set of 
    %% the RNAcentral data. 
    \label{fig:time}
    %% Each node represents a running example.
    %% The curve in the left figure shows the regression of examples from each algorithm.
  }
\end{figure} % should belong in result.tex

\section*{Results}

\begin{figure}%[h] %[h]
  \centering
  \begin{tabular}{c}
    \includegraphics[width=.4\textwidth]{figs/accu_Mathews_family_byseq_precision.pdf}
    \\[-1.45cm]
    \includegraphics[width=.4\textwidth]{figs/accu_Mathews_family_byseq_recall.pdf}
    \\[-0.2cm]
    shortest (77.3) $\xrightarrow{\makebox[4.5cm]{\text{Average Sequence Length by Family}}}$ longest (2927.4)
    \\
  \end{tabular}
\\[0.2cm]
\setlength\tabcolsep{3pt}
\begin{tabular}{c|cc|cc}
  mean  & \contrafold & \linearfoldc & \viennarna  & \linearfoldv \\
        & MFE & $b$=100 & RNAfold &  $b$=100 \\
  \hline
   PPV               &  54.80 & 56.86 (+2.1) & 50.70  & 50.92 (+0.2) \\
   Sensitivity       &  55.69 & 57.13 (+1.4) & 59.32  & 59.52 (+0.2) \\  
 \end{tabular}  
  \caption{PPV and Sensitivity (by family) on the ArchiveII dataset, comparing
    \linearfold with the corresponding baselines, \contrafoldmfe and \viennarnafold.
%% (Methods showing in same color
%%     are using the exactly same model). 
    Each column represents a family accuracy, %taking the average of the
    averaged over all sequences in that family.
%    The families are sorted ascendingly by average sequence length.%  from left to right.
%% , as
%%     the arrow represents.
    The overall accuracies are reported in the table, 
    averaging %PPV/Sensitivity 
    over all families. 
    Statistical significance is marked as %*($0.05\!\leq\! p \! < \! 0.09$),
    *($0.01 \!\leq\! p \! < \! 0.05$), and **($p\! <\! 0.01$). % represents different $p$-value.
    See Table~\ref{tab:accuracy} for detailed accuracy numbers. 
% * <david_mathews@urmc.rochester.edu> 2018-01-13T04:14:41.286Z:
% 
% > The overall accuracies are reported in the table, 
% >     averaging %PPV/Sensitivity 
% 
% 
% I don't think you should mark the P values higher than 0.05.  I think you should stick with the traditional alpha of 0.05.
% >     over all families. 
% >     Statistical significance is marked as *($0.05\!\leq\! p \! < \! 0.09$),
% >     **($0.01 \!\leq\! p \! < \! 0.05$), and ***($p\! <\! 0.01$). % represents different $p$-value.
% >     See Figure~\ref{accuracy-table} for detailed accuracy numbers.
%% Done. -- Dezhong    
% 
% ^.
    See the Methods section for details of the PPV/Sensitivity metrics and the significance testing method. % are described in 
    \label{fig:accuracy} }
\end{figure}

% impact of beam sizes
\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]%[h]
  \centering
\begin{tabular}{ccc}
\hspace{-0.1cm}
\includegraphics[width=.39\textwidth]{figs/time_modelscore_energy_Mathews.pdf} 
&
\hspace{-0.4cm}
\includegraphics[width=.33\textwidth]{figs/beamsize_nob_Mathews.pdf}
&
\hspace{-1.3cm}
\includegraphics[width=.38\textwidth]{figs/precision-recall-Mathews-contrafold.pdf}
\\
(a) & (b) & (c)
\end{tabular}  
\caption{These figures represent the trends of different variables when beam size increases.
    (a):  the internal cost, namely averaged free energy / model cost of two versions of
    \linearfold;
    (b): the number of pairs predicted (averaged by sequence) of these
    methods, comparing with Ground Truth;
    (c): PPV-sensitivity tradeoff when varying beam size.
    %% (c) and (d) choose different X/Y axis, telling different aspects of a same story.
    \label{fig:beamsize}
}
\end{figure*}
\fi

\newcommand{\subcap}[1]{\raisebox{4.5cm}{\large {#1}}}

\begin{figure*}[t]%[h]
  \centering
\begin{tabular}{cc|c}
  \setlength\tabcolsep{0.0em}
  \hspace{-0.1cm}
   \subcap{A}
  \includegraphics[width=.39\textwidth]{figs/time_modelscore_energy_Mathews.pdf} 
  &
    \hspace{-1.4cm}
   \subcap{B}
    \raisebox{0.2cm}{\includegraphics[width=.33\textwidth]{figs/beamsize_nob_Mathews.pdf}}
    \hspace{-1.cm}
  &
    \hspace{-0.2cm}
%    \raisebox{-0.5cm}{
      \subcap{E}
      \includegraphics[width=.24\textwidth]{figs/bylen_bar_precision.pdf}
%    }
  \\
%  (a) & (b) & (e)\\
  \hspace{-0.02cm}
  \subcap{C}
  \hspace{-0.13cm}
  \includegraphics[width=.40\textwidth]{figs/beam_PPV_Sens_contrafold_Mathews.pdf}
  &
  \hspace{-0.5cm}
   \subcap{D}
    \hspace{-1.1cm}
    \includegraphics[width=.42\textwidth]{figs/precision-recall-Mathews-contrafold.pdf}
    \hspace{-1.cm}
  &
    \hspace{-0.2cm}
    \subcap{F}
    \includegraphics[width=.24\textwidth]{figs/bylen_bar_recall.pdf}
%  \\
%  (c) & (d) & (f)
\end{tabular}  
\caption{Impact of beam size. A-D illustrate the trends of different variables when beam size increases.
    A:  the internal cost, namely averaged free energy / model cost of two versions of
    \linearfold;
    B: the number of pairs predicted (averaged by sequence) of these
    methods, comparing with Ground Truth;
    C: change of both PPV and Senstivity with the increasing of beam size;
    D: PPV-Sensitivity tradeoff when varying beam size;
    E-F: PPV and Sensitivity against pair distance in the ArchiveII dataset, 
    comparing \linearfoldc with \contrafoldmfe. 
    Each point represents the overall PPV/Sensitivity of all base pairs in a certain length range.
    %% (c) and (d) choose different X/Y axis, telling different aspects of a same story.
    \label{fig:beamsize}
}
\end{figure*}

\iffalse
\begin{table}[t]
\begin{tabular}{r|rr|r}
memory & \contrafoldmfe & \viennarnafold & \linearfold $b$=100\\
\hline 
%% space & \multicolumn{2}{c|}{$O(n^2)$}                   & $O(nb)$\\
%% \hline       
16G    & 27,500         & 27,500         &             \\
32G    & 32,500         & 32,500         &             \\
\end{tabular}
\smallskip
\caption{Maximum sequence length allowed by different predictors on 
machines with 16G and 32G memory.\label{tab:max}}
\end{table}
\fi

\subsection*{Efficiency and Scalability of LinearFold}
%% Building upon our previously described \linearfold algorithm, we take advantage
%% of the linear running time to predict secondary structures of RNA sequences
%% efficiently.
To demonstrate the efficiency and scalability of \linearfold,
%our linear-time prediction algorithm, 
we compare its running time with the conventional cubic-time prediction algorithms
used in the baseline systems, \contrafold and \viennarnafold.
Figure~\ref{fig:time} shows the results on two datasets: 
(a) the ArchiveII dataset \cite{sloma+mathews:2016}, a diverse
set of RNA sequences with known structures (see details in the Methods
section and Table~\ref{tab:accuracy}),
and (b) a (sampled) subset of RNAcentral \cite{rnacentral:2017}, 
a comprehensive (meta-)set of 
%non-coding RNA 
ncRNA
sequences from many databases.
While the ArchiveII set contains sequences of length 3,000 or less,
the RNAcentral set has many much longer sequences, with the longest being 244,296 \nts 
(Homo Sapiens Transcript NONHSAT168677.1, from the NONCODE database \cite{noncode:2016}).
We use a machine with 3.40GHz Intel Xeon CPUs and 32G memory, running Linux;
all programs are written in C/C++ compiled by GCC 4.9.0.
%% We first test on the ArchiveII dataset (more details described in later
%% section), comparing to previous approaches, namely \contrafoldmfe and \viennarna
%% RNAfold.
% * <david_mathews@urmc.rochester.edu> 2018-01-13T04:02:08.620Z:
% 
% > (more details described in later
% > section)
% 
% Please cite:
% Sloma, M.F., & Mathews, D.H. (2016). Exact calculation of loop formation probability identifies folding motifs in RNA secondary structures. RNA. 22, 1808-1818
% 
% ^.
%% Done -- Dezhong

%, comparing to previous approaches, namely \contrafoldmfe and \viennarnafold.

%% We further aim to predict structures on longer RNA sequences, with
%% length ranging from $10^3$\nts to $10^5$\nts, as we randomly generate RNA sequences
%% based on the distribution of nucleotides, and run experiments using these
%% approaches.
%% Results of these experiments (choosing $b$=100 as the beamsize in \linearfold,
%% the default in all experiments below, if not specified)
%% are represented in Figure~\ref{time-scatter}. 
%% =======
%% We further aim to predict structures on longer RNA sequences, with
%% length ranging from $10^3$\nts to $10^5$\nts, as we randomly generate RNA sequences
%% based on the distribution of nucleotides, and run experiments using these
%% approaches.
%% Results of these experiments (choosing $b$=100 as the beamsize in \linearfold,
%% the default in all experiments below, if not specified)
%% are represented in Figure~\ref{fig:time}. 
%% >>>>>>> 0a233712acca153b13df872d32109a7f6c9675b1
% * <david_mathews@urmc.rochester.edu> 2018-01-13T04:08:19.000Z:
% 
% > Figure~\ref{time-scatter}.
% I couldn't find the caption for this figure to edit the text, sorry.
% I suggest changing "speed comparisons" to "Runtime comparisons".  Also, change "Mathews dataset" to "set of RNA sequences with known structure".
% Also, the y-axis needs "sentence" changed to "sequence".
% 
% I don't see that the manuscript details the OS, compiler, and CPU for the timing.  I think this caption could contain these details.
% 
% ^.
% We have also compared \linearfold with other approaches ({\it SI Appendix},
% Figure 1). %% ADD IT OR NOT?
% Done - Liang.

Figure~\ref{fig:time} A confirms that \linearfold's
%runs in time linear in sequence length,
running time scales linearly with the sequence length,
while the two baseline systems scale superlinearly, with an empirical runtime of $O(n^{2.6})$
determined by curve fitting.
Figure~\ref{fig:time} B reconfirms this fact
on much longer sequences (in log-scale),
and for a sequence of $\sim$10,000 \nts
(e.g., the HIV genome),
\linearfold (with the default beam size of $b$=100) takes only 7 seconds
while the baselines take 4 minutes.
For sequences of length 32,753,
our \linearfold takes only 23 seconds
while \contrafold takes 2 hours and RNAfold 1.7 hours.
This clearly shows the advantage of our linear-time prediction algorithm
on very long %non-coding RNAs.
ncRNAs.

In addition, \linearfold also has an advantage on memory usage that leads to better scalability on extremely long sequences.
The baseline cubic-time algorithms
require memory space that scales {\em quadratically} with sequence length,
because intuitively they need to figure out the best scoring or minimum free energy structure
for every substring $[i, j]$ of the entire sequence.
This means you need 4x memory if your sequence length doubles.
%Due to this limitation, on our 32GB-memory machine, 
In addition,
due to a design deficiency,
neither \contrafoldmfe or \viennarnafold 
runs on any sequence longer than 32,767 \nts.
On the other hand, \linearfold not only takes linear time,
but also uses linear memory, 
without the need for the two-dimensional table of size $O(n^2)$.
As a result, \linearfold is able to process the longest sequence in RNAcentral (244,296 \nts),
taking less than 3 minutes.
%(which is even faster than the baselines' runtimes on sequences of $\sim$10,000 \nts).
In fact, \linearfold even scales to sequences of 10,000,000 \nts on our 32GB-memory machine.

%% Because \linearfold maintains a constant number of states in each step regardless of
%% the input RNA sequence length, it achieves a linear running time comparing to
%% the rapidly increasing time of every previous approach
%% (where calculating the optimal folding energy for all the subsequences is required). 
%% As expected, this time difference becomes more pronounced as the sequence length
%% increases, where \linearfold with a beam width of $b$=100 achieves 2.75 times
%% faster on $n$=3000, and 30 times faster on $n$=$10^5$ (e.g., the TTN-202 transcript \cite{robinson+:2005}
%% \footnote{The online reference is available 
%%   \href{http://www.ensembl.org/Homo_sapiens/Transcript/Summary?g=ENSG00000155657;r=2:178525989-178807421;t=ENST00000342992}{here}.})
%% than the fastest previous approach. 
%% As a result, \linearfold becomes applicable and much more efficient in
%% predicting long RNA sequences while previous approaches suffer from a long
%% running time.
                                        
\iffalse
%% These results show that the running time of our algorithm is linearly increasing
%% with the sequence length $n$, different from the previous two algorithms.
%% Benefiting from the sparsity of possible nucleotides pairings, the bottom-up
%% dynamic programming based algorithms has the $O(n^{2.6})$ actual running time
%% instead of cubic. However, \linearfold starts to outperform as the sequence
%% length increases, as the running time of the previous approaches increase
%% rapidly. As shown in the figure, all approaches have a similar running time when the RNA
%% sequence length is relatively small ($<700nt$), while our algorithm is about
%% $2.75$ times faster than \contrafoldmfe, and about $4$ times faster than \viennarna
%% RNAfold for 23S rRNA sequences (towards the right, with average length around
%% $2927nt$). 

%% This shows a great potential of our algorithm that for our left-to-right
%% prediction on an RNA sequence, the time required to process a single nucleotide
%% is no longer related to the length of the prefix, while for previous approaches,
%% increasing the sequence length even by one, would cost a huge additional amount of
%% time. 

%% To further investigate the efficiency, we randomly generate a set of RNA
%% sequences with length from $1,000nt$ to $10,000nt$, using the same nucleotide
%% distribution of the actual RNA sequences. 
%% Figure~\ref{time-long} is a log-log plot showing the experimental results.

%% Taking a randomly generated sequence with about $10,000nt$ as an example, both
%% \viennarnafold and \contrafoldmfe need more than $200$ seconds on average to get
%% the predicted structure, while the running time of \linearfold is around $7.11$
%% seconds.

\fi

\subsection*{Accuracy of LinearFold}

%% After showing the efficiency of our proposed \linearfold algorithm,
%% we further prove that \linearfold leads to more accurate RNA structure predictions
%% comparing to previous approaches, even with a significantly reduced amount of
%% time. 
%We now compare
We next compare
the prediction accuracies of \linearfold
and the two baseline systems,
reporting both Positive Predictive Value (PPV; the fraction of predicted pairs in the known structure) and Sensitivity (the fraction of known pairs predicted) 
on each RNA family in ArchiveII dataset.
%With the defau $b$=100, 
%% Figure~\ref{fig:accuracy}
%% shows the results on the ArchiveII dataset %(same as all experiments below, if not
%% % =======
%% %% we further demonstrate that \linearfold provides more accurate RNA structure predictions
%% %% comparing to previous approaches, even with a significantly reduced 
%% %% runtime. Choosing b=100, we report our experimental results in Figure~\ref{histogram-accuracy}.
%% %% We use the dataset of diverse RNA families with known structure (same as all experiments below, if not
%% %% >>>>>>> 2eb31642b206083a2f9ffb0de62c59cd26ca2ffa
%% %specified),
%% reporting both Positive Predictive Value (PPV; the fraction of predicted pairs in the known structure) and Sensitivity (the fraction of known pairs predicted) 
%% on each RNA family. 
%% We compared \contrafoldmfe (with a machine-learned model) 
%% with its linear-time version, \linearfoldc,
%% and \viennarnafold (with a thermodynamic model,
%% with energy parameters from \cite{mathews+:1999})
%% with its linear-time version, \linearfoldv.
We also tested statistical significance using a paired, two-tailed
$t$-test, following previous work \cite{xu+:2011}.
% * <david_mathews@urmc.rochester.edu> 2018-02-01T05:00:52.783Z:
% 
% Please fix capitalization in title of reference 49, Xu et al.  "RNA" not "rna".
% 
% ^.
% * <david_mathews@urmc.rochester.edu> 2018-01-13T04:21:47.475Z:
% 
% > following previous work\cite{hajiaghayi+:2012}.
% Please change citation to:
% Xu, Z., Almudevar, A., & Mathews, D. H. (2012). Statistical evaluation of improvement in RNA secondary structure prediction. Nucleic Acids Research. 40, e26. 
% 
% The reference you cite is also good work, but they used bootstrapping to assess significance.
% 
% ^.
% Done -- Dezhong
% We further prove that \linearfold leads to more accurate RNA structure
% predictions comparing to previous approaches, even with a significantly reduced
% amount of time (Figure~\ref{histogram-accuracy}).
Figure~\ref{fig:accuracy} shows that
%, overall, 
\linearfoldc improves PPV and Sensitivity over \contrafold by +2.1\%/+1.4\% (absolute)%,
when averaged across all families.
This is surprising %as
because
\linearfold produces more accurate structures
using a fraction of runtime.
%% comparing to previous approaches, even with a significantly reduced amount of
%% time. 
Individually, \linearfoldc is significantly more accurate in both PPV/Sensitivity
on three families: Group I Intron, 16S and 23S ribosomal RNAs,
with the last two being the longest families in this dataset.
16S rRNAs have an average length of 1548 \nts and +3.89\%/+3.08\% absolute improvement in PPV/Sensitivity,
and 23S rRNAs have an average length of 2927 \nts and +14.00\%/+9.98\% absolute improvement. 
%This is even more surprising, that
Even more surprising, 
\linearfold's improvement in accuracy is more pronounced on longer sequences.
Accuracies are also improved by \linearfoldv over \viennarnafold, 
but the difference is smaller (overall +0.2\%/+0.2\% absolute improvement in PPV/Sensitivity).
Individually, the improvement is significant on both PPV/Sensitivity on two families,
Group I Intron and 16S rRNA.
%%  indicates that our \linearfold algorithm
%% is 

%% Comparing \contrafoldmfe with \linearfoldc, while the latter improves the prediction
%% quality slightly on most RNA families, we improve significantly on longer RNA families,
%% namely 16S (average 1548{\em nt}s, +3.89\%/+3.08\% on PPV/Sensitivity) and 23S Ribosomal
%% RNAs (average 2927{\em nt}s, +14.00\%/+9.98\%). This surprisingly shows that our
%% algorithm could predict better structures on harder tasks.

% According to Figure~\ref{histogram-accuracy}, while the prediction quality has
% been improved on most of the RNA families, we observe that our improvements are
% much more significant on longer RNA families, especially 16S (C:+3.89\%/+3.08\%
% on PPV/Sensitivity; V:+1.46\%/+1.56\%) and 23S Ribosomal
% RNAs 

% Despite using a reduced amount of
% running time, \linearfold achieves a better overall accuracy, improving prediction
% quality on both thermodynamic models and machine learned models.
% Moreover, the improvements are more represented on machine learned models
% (+1.9\%/+1.4\% on PPV/Sensitivity) than on
% thermodynamic models (+0.3\%/+0.5\%).

% Moreover, the improvements of prediction are more represented in longer RNA families. 

% Comparing \linearfoldc with \contrafoldmfe, we got 1.9\% / 1.4\%
% improvements on PPV/Sensitivity. 

% as it
% would restrict the output structure survives in every single step from left-ro-right,
% rather than simply calculating the global optimal structure from the model. 

% As expected, the improvements of prediction are more represented in longer RNA
% families, in which each step contains more states, that our beam pruning can
% prune out more low-scoring states towards heuristics.

%As a by-product, \linearfold 

% Specifically, our beam search would not make much difference in predicting
% shorter RNA sequences as the number of merged states in one step is very
% limited, but when the sequence length increases, more low-scoring states would be
% pruned out in each step, which leads to more heuristics towards the predicted structure, 

% when
% predicting shorter RNA sequences, our beam search does not prune out 

% As expected, the improvements are much bigger in longer RNA families, as more
% restrictions are enforced in more prediction steps. 

\iffalse
While \linearfold outperforms slightly among all the sequences, the general trend
by family shows that the difference in both PPV/Sensitivity are much bigger with
longer RNA families. On shorter RNA families (like tRNA($77.2nt$) and 5S
rRNA ($118.8nt$)), both PPV and Sensitivity are almost the same,  while a
large improvement can be observed on 16S rRNA ($1547.9nt$) and 23S rRNA
($2927.4nt$). 

These results also show that our accuracy improvements are much higher when
using the machine-learned model (\linearfoldc over \contrafoldmfe) than the
thermodynamic model (\linearfoldv over \viennarnafold). Generally, the \viennarna
thermodynamic model is much more stable, while the \contrafold
machine-learned model is quite sensitive to hyperparameters. For example, the beamsize in
\linearfold helps us balance local and global competing objectives. 

We also observe that in most of the RNA sequences, the thermodynamic model tends
to predict a lot more base pairs than the machine-learned one in
general. This leads to the Sensitivity of methods using a thermodynamic model being
generally higher than those that use a machine-learned model. By adapting \linearfold,
the low Sensitivity of machine-learned models have been improved to be
comparable to thermodynamic ones. 
\fi

% This figure also shows that our improvements over previous methods are much more
% obvious using the machine-learned model than the thermodynamic model. As
% the \viennarna thermodynamic model is much more stabalized, it is much harder to
% make a difference over it.  

%% \contrafold improve, more than \viennarna

\iffalse%^%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure} %[h]
  \centering
  \hspace{-1.cm} 
  \begin{tabular}{cc}
  \hspace{-.4cm} 
      \includegraphics[width=.28\textwidth]{figs/bylen_bar_precision.pdf}
    & \hspace{-1.1cm}
      \includegraphics[width=.28\textwidth]{figs/bylen_bar_recall.pdf}
      \\[-0.2cm]
  \end{tabular}
  \caption{PPV and Sensitivity against pair distance in the ArchiveII dataset, 
    comparing \linearfoldc with \contrafoldmfe. 
    Each point represents the overall PPV/Sensitivity of all base pairs in a certain length range.
  \label{fig:long-range} }
\end{figure}
\fi

\begin{figure*}[t]% [h]
  \centering
  \begin{tabular}{p{0.1cm}|c|c|c}
    % \begin{subfigure}
    %   \centering

&    Group I Intron \cmirabilis (526\nts, 143 \pairs)
    &
      16S rRNA \apyrophilus (1564\nts, 468 \pairs)
    &
      23S rRNA \ecoli (2904\nts, 830 \pairs)
    \\
    \hline
\rot{\hspace{1.5cm}\contrafoldmfe}    
 &   \includegraphics[width=.3\textwidth]{figs/new_4_contrafold.pdf} % grp1 a.I1.e.C.mirabilis.C1.SSU \contrafoldmfe: $PPV=38.96, Sens=41.96, pairs=154$.
    &
    \includegraphics[width=.3\textwidth]{figs/16s_8_contrafold.pdf} % 16s subtilis \contrafoldmfe: $PPV=43.10, Sens=44.35, pairs=464$.
    &
    \includegraphics[width=.3\textwidth]{figs/23s_4_contrafold.pdf} % 23S Ecoli \contrafoldmfe: $PPV=47.49, Sens=48.92, pairs=855$.
    % \end{subfigure}

    \\

 &   \ppv: 38.96, \sens: 41.96, \pairs: 154.
    &
    \ppv: 53.20, \sens: 58.55, \pairs: 515.
    &
    \ppv: 47.49, \sens: 48.92, \pairs: 855.
    \\[0.3cm]
\hdashline

%    \hline %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % \begin{subfigure}
    %   \centering
\rot{\hspace{1.5cm} \linearfoldc $b$=100}
 &   \includegraphics[width=.3\textwidth]{figs/new_4_beam100.pdf} % grp1 a.I1.e.C.mirabilis.C1.SSU \linearfoldc : \ppv: 67.74, \sens: 73.43, \pairs: 155.
    &
    \includegraphics[width=.3\textwidth]{figs/16s_8_beam100.pdf} % 16s subtilis \linearfoldc: \ppv: 66.74, \sens: 68.51, \pairs: 463.
    &
    \includegraphics[width=.3\textwidth]{figs/23s_4_beam100.pdf} % 23S Ecoli \linearfoldc $b=100$: \ppv: 69.94, \sens: 67.83, \pairs: 805.
    % \end{subfigure}
    \\

  &  \ppv: 67.74, \sens: 73.43, \pairs: 155.
    &
    \ppv: 61.49, \sens: 65.17, \pairs: 496.
    &
    \ppv: 69.94, \sens: 67.83, \pairs: 805.
    \\

    % \contrafoldmfe: \ppv: 47.49, Sens=48.92, pairs=855$.
    
    % &

    % \linearfoldc $b=100$: \ppv: 69.94, Sens=67.83, pairs=805$.

    % \\

    % % \begin{subfigure}
    % %   \centering
    %   \includegraphics[width=.3\textwidth]{figs/23s_4_vienna.pdf}
    % % \end{subfigure}

    % &
      
    % % \begin{subfigure}
    % %   \centering
    %   \includegraphics[width=.3\textwidth]{figs/23s_4_linearvienna.pdf}
    % % \end{subfigure}

    % \\

    % \viennarnafold: $P=52.34, R=57.83, pairs=917$.
    
    % &

    % \linearfoldv $b=100$: $P=56.14,R=62.77, pairs=928$.

    % \\
    
  \end{tabular}
  \caption{Circular plots of 3 RNA sequences (selected from 3 different RNA
    families ) comparing \contrafoldmfe with \linearfoldc.
  A blue arc represents a correctly predicted pair, a red arc represents an
  incorrectly predicted pair, while a light gray arc represents a based pair
  miss predicted. Each plot uses the clockwise order of the RNA sequence from
  the top.
  These 3 examples are picked from 3 different RNA families that the performance
  of \linearfoldc is improved significantly comparing to \contrafoldmfe. 
  \label{fig:circular}}
\end{figure*}

\subsection*{Impact of Beam Size}

%In the above subsections, 
Above we used $b$=100 as the default beam size. Now we
investigate the impact of different beam sizes. We first study the impact of
search quality. Since our \linearfold algorithm uses approximate search instead
of exact search, we use the difference between exact search free energy and our
returned free energy as the measure of search quality -- the closer they are,
the better our search quality. We can see from Figure~\ref{fig:beamsize}
A that the search quality is getting closer when the beam size increases, and 
\linearfold achieves similar model cost / free energy using the default beam
size. 
Similarly, Figure~\ref{fig:beamsize} B plots the number of pairs predicted, at
each beam size. It shows that \viennarna model tends to overpredict, while the
\contrafold model underpredicts. Also, although our algorithm always underpredicts
compared to exact predictions in either model, we predict almost the same number of base pairs
as each model when using the default beam size. The mean difference is 0.29(\contrafold)/0.01(\viennarna) pairs
when $b$ = 100.


%% Since our linear algorithm is approximate, 
%% so we use the different between the exact search free energy and our returned
%% free energy
%% as the measure of search quality.
%% the closer we are, the better search quality it is. 

% As a beam-search-based incremental prediction algorithm, the
% prediction %quality
% performance 
% of \linearfold is highly impacted by the beam size, the maximum number of
% states allowed in each step of the algorithm.
% We investigated different variables reflecting prediction 
% %quality
% performance 
% and report their trends by the change of beam size, showing in Figure~\ref{fig:beamsize}.

% is "search quality" below the right expression here? In a way these are both "objective functions" for the minimization procedures, so perhaps a term like that? 
% Figure~\ref{fig:beamsize} (a) plots search quality (model cost in machine-learned
% models; free energy in thermodynamic models) against beam size. We can see
% \linearfold achieves similar model cost / free energy using a very small beam
% (e.g., b=100), using much smaller search space than the previous approaches
% (i.e., much faster).

% Similarly, Figure~\ref{fig:beamsize} (b) plots number of pairs predicted against
% beam size. This also verifies the thermodynamic models tend to achieve much higher
% Sensitivity and lower recall, comparing with the machine learned models, since
% it predicts more pairs overall.

%% trade-off;
%% peak at 120
%% very consistent in b=100~150

Figure~\ref{fig:beamsize} C plots PPV and Sensitivity as a function of beam size~$b$.
\linearfoldc outperforms  \contrafoldmfe in both PPV and Sensitivity 
with $b\ge 75$ (though it will converge to \contrafoldmfe when $b\rightarrow +\infty$),
and \linearfoldc's PPV/Sensitivity are stable with $b\in [100,150]$.
Figure~\ref{fig:beamsize} D shows the tradeoff of PPV and Sensitivity of
\linearfold, with the change of the beam size. It starts with the increasing of
both PPV and Sensitivity, reaches the peak at $b$=120, and falls until
converging to exact search. Although the peak happens when beam size is 120, we
can see that the performance \linearfold is consistent when its beam size is
in [100,150], as both PPV/Sensitivity stays almost the same. 

% From Figure~\ref{fig:beamsize} (c) and (d), we can observe the trends of PPV,
% Sensitivity and the search quality of \linearfoldc, by the change of the beam
% size. The result confirms our predictions converge to the corresponding baseline
% when beam increases to infinite. It also reveals the changes of PPV/Sensitivity
% become very small when b$\geq$100, showing the most of the prediction errors
% could be solved by a smaller beam size. (d) also confirms our b=100 choosing is
% very general, not cherry-picked by the evaluation results. 

% While ``outer score'' (PPV/Sensitivity) reflects the performance of predicted structures
%  evaluated by the Ground Truth, the ``inner score'' (model cost in
% machine learned models; free energy in thermodynamic models) evaluates the
% prediction quality of them by the model itself. 

\subsection*{Accuracy Improvements on Long-Range Base Pairs}

%We further arranged our performance by the base-pair distance over the
%ArchiveII dataset and observe the evaluation metrics. 
We further evaluated the effect of the distance between base paired-nucleotides on prediction performance.
As shown in Figure~\ref{fig:beamsize} E and F,
when predicting long-distance pairs, 
\linearfold can outperform previous approaches in both PPV and Sensitivity. %, 
%when predicting long-distance pairs. 
% %Generally,
% One would expect that
% keeping the $b$-best states in each step instead of all states would generally
% lead the 
% %prediction 
% prediction 
% % I'm changining all occurences of "optimums" to "optima" here -DH
% of locally optimal structures rather than  
% globally optimal structures, while for lower values of $b$, more local base pairs are predicted.
% % * <david_mathews@urmc.rochester.edu> 2018-02-01T05:16:00.791Z:
% % 
% % "while for lower values of $b$, more local base pairs are predicted."
% % I am not sure what you mean to convey here.  Are you saying that at b=50, this is the case that more local pairs are predicted?  I think this needs to then be a separate sentence.
% % 
% %
% %% Done. -- Dezhong
% ^.
%That leads to a concern if \linearfold could predict long-distance pairs more
%accurately than previous methods. These results have shown that
%for nucleotide pairs in long distances, \linearfold avoids predicting large
%numbers of incorrect base pairs, while still catching all the correct
%base pairs predicted by the previous methods.
Contrary to the concern that \linearfold would not predict as accurately for long-distance pairs, it continues to outperform previous methods even at pairing distances over 500 nt. 
Detailed comparisons between \linearfoldv and \viennarnafold in PPV,
Sensitivity, and prediction quality, are in the Supporting Information. 

%We also observe that although increasing beamsize $b$ would almost guarantee
%improve the performance, the improvement becomes very small when
%$b>100$ for this model.
% We also observe that the improvement in performance from increasing the beamsize $b$ becomes very small for this model when $b>100$. 

% While the predictions are reduced slightly as the algorithm
% tries to predict more base-pairs, it doesn't succeed very much. 

\subsection*{Example Predictions: Group I Intron, 16S and 23S rRNAs}

We visualized the predicted secondary structure of 3 examples from different RNA
families, Group I Intron \cmirabilis, 16S rRNA \apyrophilus, 23S rRNA \ecoli, 
% * <david_mathews@urmc.rochester.edu> 2018-02-01T05:22:20.438Z:
% 
% Here and in Figure 5, be sure that you italicize genus and species names.  Also, I think pyrophilus is a species, but Mirabilis is a genus?  Please give names as "Genus species" where the genus is capitalized and species is not capitalized.  This is the convention for naming species.
% 
% ^.
comparing \linearfoldc with \contrafoldmfe (Figure~\ref{fig:circular}). 
% I thought "clearly" here is a bit strong. We know these are sort of picked examples, so maybe this should be toned down? 
%The circular plots clearly show our performance improvement, by both predicting
The circular plots show our performance improvement, by both predicting
more base pairs correctly, and %reduce
reducing
incorrect predictions. 
This visualization also 
%proves that our \linearfold is better at handling
demonstrates \linearfold's improved prediction of 
long-distance base pairs than the baseline, as shown in Group I Mirabilis (bottom half,
pair distance ~250), 16S \apyrophilus (left part, ~550), 23S \ecoli (left part,
~600). 
Fig.~\ref{fig:si-circle} shows
the corresponding results comparing \linearfoldv with \viennarnafold.
%, including the
%% traditional collapsed-format plots for these structures, 
%% and the structures of
%. 
We also built a \href{http://web.engr.oregonstate.edu/~liukaib/demo_json+svg.html}{web demo}
visualizing results from all sequences in these three families.\footnote{\url{http://web.engr.oregonstate.edu/~liukaib/demo_json+svg.html}}


% Generally, there is about a $20\%$ accuracy improvement from \contrafoldmfe to
% \linearfoldc, while about a $4\%$ accuracy improvement on the \viennarnafold
% model. This proves the thermodynamic model is a lot more stabalized than the
% machine-learned model in general.

% For the machine-learned model, \linearfold tends to significantly reduce the
% incorrectly predicted base-pairs, especially for long-distance pairs. At the same
% time, a decent number of correct base pairs are found by the improved model,
% which leads to an improvement on both PPV and Sensitivity.

% This observation stays the same for the thermodynamic model, while the
% improvement is smaller compare to the previous one.
% The predicted structures have shown another nice property of \linearfold that
% although a large number of possible structures have been tuned during the
% left-to-right incremental search, we still keep the possibility of predicting
% long-distance base-pairs alive until the end, such that we correctly predict all
% the longest base-pairs (about $2900nt$) using significantly less time, with improved PPV
% and Sensitivity in the entire sequence. 

% We provide more detailed results in the appendix, including more details of
% efficiency and accuracy comparisons, tuning of hyperparameters, the different
% properties of the two models, and predicted structures of additional sequences. 

% \begin{SCfigure*}[\sidecaptionrelwidth][h]
% \begin{figure*}%[\sidecaptionrelwidth][h]
% \centering
% \subfigure[Performance of \linearfold by family.]{\label{fig:histogram1}\includegraphics[]{figs/accu_Mathews_family_byseq}}
% \subfigure[Performance of \linearfold over \contrafold/\viennarna by family.]{\label{fig:histogram2}\includegraphics[]{figs/accudiff_family_byseq}}
% \caption{}
% \label{fig:histogram}
% \end{figure*}

% Figure~\ref{fig:prelim} compares our incremental $O(n)$ algorithm with 
% traditional $O(n^3)$-time Zuker algorithms,
% on the pseudoknot-free subset (1,068 sequences) of CompaRNA, using the \contrafold model
% trained from the 151-sequence Rfam dataset.
% The baseline (Zuker) is a reasonably faithful reimplementation of the highly optimized 
% code of \contrafold (Viterbi mode, analogous to minimum free energy or MFE mode in other software).
% Part (a) plots search quality (model score) against search space (number of states explored),
% at various beam sizes. 
% %% Note that CKY is also with beam pruning, but 
% %% beaming per $[i,j]$ span instead.
% We can see that linear-time DP can achieve similar model score 
% using $b=100\sim500$, using much smaller search space than Zuker (i.e., much faster).
% %  at the same level of search quality;
% %for example, ours at $b=2000$ is similar in quality to CKY at $k=50$, but explores only 1/4 of states.
% Similarly, part (b) plots accuracy (defined as F-1 measure between Sensitivity and positive predictive value\footnote{Sensitivity = $\frac{\text{\# correctly predicted base pairs}}{\text{\# ground-truth base pairs}}$,
% positive predictive value = $\frac{\text{\#correctly predicted base pairs}}{\text{\# predicted base pairs}}$,
% and F-1 score is the harmonic mean between them.}) %$\frac{2 \cdot \mathrm{Sensitivity} \cdot \mathrm{ppv}}{\mathrm{Sensitivity} + \mathrm{ppv}}$.})
% against wall-clock time, and even more strikingly, %reflects the same trend.
% linear DP with $b=100$ scores higher than exact Zuker but using only 1/5 of time.
% Part (c) verifies that our predictor scales linearly, and Zuker %scales superlinearly
% has an empirical complexity of $n^{2.5}$ (due to optimizations in the style of \contrafold). %$in Section~\ref{sec:proposed}).
% More surprisingly, part (d) shows that the relative advantage of our linear-time predictor 
% over exact Zuker
% is even more pronounced for base pairs that are farther away from each other in the sequence,
% suggesting that our method is better for those hard-to-predict long-distance dependencies.
% %although the prediction accuracy degrades with larger base pair distance 
% Part (e) compares our linear-time DP at $b$=100 with other major software,
% including \contrafold MEA mode (maximum expected accuracy,
% which is about 2 points more accurate than the Viterbi or MFE mode),
% \viennarnafold, and \rnastructure.
% Ours is the fastest in speed, and second in terms of accuracy (only after \contrafold MEA,
% which we will address in  WHICH CHAPTER).
% Part (f) is a log-log plot of speed vs.~length %of these software 
% on longer, randomly generated, sequences between 1,000 and 10,000 nts.
% It confirms that our predictor is linear time, and is orders of magnitude faster 
% than existing software on extremely long sequences; for example, 
% on a sequence of 10,000 nts (similar in length to the HIV genome),
% our method takes {\bf 10 seconds} whereas \rnastructure takes {\bf 4 hours}.


==> significance.tex <==
Fast and accurate prediction of RNA secondary structures 
(the set of canonical base pairs)
is an important problem, 
because RNA structures reveal crucial information about their functions.
Existing approaches can reach a reasonable accuracy 
for relatively short RNAs %shorter than 800 nucleotides, 
but their running time scales almost cubically with sequence length,
which is too slow for longer RNAs.
We develop the first linear-time algorithm for RNA secondary structure prediction.
%Our algorithm works for both thermodynamic and machine learned models,
Surprisingly, our algorithm not only runs much faster,
but also leads to higher overall accuracy % over all families 
on a diverse set of RNA sequences with known structures,
where the improvement is significant for long RNA families such as
%significantly higher accuracies for the longest RNA families such as 
%% and more interestingly, this improvement is significant on long RNA families such as
16S and 23S Ribosomal RNAs.
More interestingly, it also more accurate for long-range base pairs.

%without loss of accuracy.
%% many RNA sequences are not translated to proteins (non-coding RNAs)
%% and instead have intrinsic functions; 

%%  non-coding RNAs. 
%% (e.g., the HIV genome has $\sim$10,000 nucleotides).
%% to be useful experimentally
%% While experimental assays still constitute the most reliable way to determine
%% such structures, they are prohibitively costly and slow; 
%% therefore computational prediction provides an attractive alternative. 
%% In this direction, 

%and we call these RNA sequences noncoding RNA
%% , which is useful in many
%% applications ranging from noncoding RNA detection to the design of oligonucleotides for knockdown of message.
%various studies have greatly improved the accuracy of prediction, but there is
%not enough attention on the speed of prediction.

%% that is high enough 
%% to be useful in developing hypotheses that can be tested experimentally,

%All existing approaches to this problem use a dynamic programming algorithm 
%\cite{mathews+turner:2006,washietl+:2012}.  
%% On average, 73\% of known base pairs are correctly predicted in benchmarks of accuracy for sequences shorter than 800 nucleotides \cite{mathews+:2004,lu+:2009,bellaousov+mathews:2010}.  
%% This accuracy is high enough to be useful in developing hypotheses that can be tested experimentally.  But these methods have time complexity ranging from $O(n^3)$ to $O(n^6)$, where $n$ is the sequence length, which is too slow for long ncRNAs ($n\!>\!1,000$).  This proposal would address this bottleneck in analysis by providing accurate structure prediction with {\bf linear-time complexity}, using the PI's recent breakthroughs in natural language processing \cite{huang+sagae:2010}.

% from Mathews, used in the R01 proposal

\iffalse
{\bf RNA is Critical to Cellular Function.}  
Over the last three decades, we have become increasingly aware that RNA is actively involved in Biology.  Many RNA sequences have intrinsic functions, without being translated to proteins, and we call these RNA sequences noncoding RNA (ncRNA) \cite{eddy:2001}.  
ncRNA sequences catalyze reactions \cite{doudna+cech:2002,scott:2007},  
regulate gene expression \cite{storz+gottesman:2006,wu+belasco:2008,serganov+nudler:2013},  provide site recognition for proteins \cite{bachellerie+:2002,wahl+:2009} and serve in trafficking of proteins \cite{walter+blobel:1982}.  It is known that many regions in genomes are transcribed, suggesting there are yet a large number of unknown ncRNA sequences, and new ncRNAs are being reported regularly \cite{birney+:2007}.  A new frontier is the discovery and characterization of long noncoding RNAs \cite{johnsson+:2014}.  Furthermore, the dual nature of RNA as both a genetic material and functional molecule led to the RNA World hypothesis, that RNA was the first molecule of life \cite{gilbert:1986},  and this dual nature has also been utilized to develop in vitro methods to evolve functional sequences \cite{joyce:1994}. Finally, RNA is an important drug target and agent \cite{sucheck+wong:2000,sazani+:2002,crooke:2004,childs-disney+:2007,gareiss+:2008,castanotto+rossi:2009,palde+:2010}.

{\bf Overview of RNA Structure.}
RNA structure is hierarchical \cite{tinoco+bustamante:1999}.  The primary structure is the covalent structure encoded in the nucleotide sequence.  The secondary structure is the set of canonical base pairs (A-U, G-C, and G-U; Fig.~\ref{fig:pseudoknot}).  The tertiary structure is the 3D structure and the full set of molecular contacts.  Secondary structure generally forms faster \cite{zarrinkar+williamson:1994,woodson:2000} and is more stable \cite{crothers+:1974,banerjee+:1993,onoa+:2003} than tertiary structure.  Therefore, secondary structure can be accurately predicted independently of tertiary structure.

{\bf Prediction of RNA Secondary Structure.}
The most popular approach to RNA secondary structure prediction is free energy minimization with a dynamic programming algorithm \cite{mathews+turner:2006,washietl+:2012}.  On average, 73\% of known base pairs are correctly predicted in benchmarks of accuracy for sequences shorter than 800 nucleotides \cite{mathews+:2004,lu+:2009,bellaousov+mathews:2010}.  This accuracy is high enough to be useful in developing hypotheses that can be tested experimentally.  But these methods have time complexity ranging from $O(n^3)$ to $O(n^6)$, where $n$ is the sequence length, which is too slow for long ncRNAs ($n\!>\!1,000$).  This proposal would address this bottleneck in analysis by providing accurate structure prediction with {\bf linear-time complexity}, using the PI's recent breakthroughs in natural language processing \cite{huang+sagae:2010}.
\fi

